Accelerating Large-Scale Reasoning Model Inference with Sparse Self-Speculative Decoding

Reasoning language models have demonstrated remarkable capabilities on challenging tasks by generating elaborate chain-of-thought (CoT) solutions. However, such lengthy generation shifts the inference bottleneck from compute-bound to memory-bound. To generate each token, the model applies full attention to all previously generated tokens, requiring memory access to an increasingly large KV-Cache. Consequently, longer generations demand more memory access for every step, leading to substantial pressure on memory bandwidth. To address this, we introduce SparseSpec, a speculative decoding framework that reuses the same model as the draft and target models (i.e., self-speculation). SparseSpec features a novel sparse attention mechanism, PillarAttn, as the draft model, which accurately selects critical tokens via elegantly reusing information from the verification stage. Furthermore, SparseSpec co-designs self-speculation with three system innovations: (1) a unified scheduler to batch token drafting and verification, (2) delayed verification for CPU/GPU overlap, and (3) dynamic KV-Cache management to maximize memory utilization. Across various models and datasets, SparseSpec outperforms state-of-the-art solutions, with an up to 2.13x throughput speedup.

==> Figures/fig-eval-breakdown.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig-eval-breakdown.pdf}
    \caption{Breakdown of generation time when serving \dpsk{}-\lm{}-8B on H100 with \sys{} and vLLM.
Results show that \sys{} greatly reduces the memory bandwidth bottleneck, without incurring computational overhead.\fixme{}}
    \label{fig-eval-breakdown}
\end{figure}


==> Figures/fig-motivation-speculative.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig-motivation-speculative.pdf}
    \caption{Qualitative comparison between \sys{} and existing speculative decoding methods.
Existing methods either have high training and deployment efforts or fail to deliver high speedups due to a low acceptance rate.
\sys{} uses \sspec{} to achieve high throughput gains without training.}
    \label{fig-motivation-speculative}
\end{figure}


==> Figures/fig-placeholder.tex <==
\begin{figure}[!t]
    \centering
    \vspace{-2mm}
    \includegraphics[width=0.95\linewidth]{Figures/fig-placeholder.pdf}
    \caption{\fixme{placeholder.} Compute density of requests with different input/output lengths (Qwen3-1.7B on an A100 80GB GPU) varies drastically.
    }
    \vspace{-2mm}
\end{figure}


==> Makefile <==
# Makefile for building LaTeX document with pdflatex

# Main document name (without .tex extension)
MAIN = _main

# LaTeX compiler
LATEX = pdflatex
BIBTEX = bibtex

# LaTeX compiler flags
LATEX_FLAGS = -interaction=nonstopmode -halt-on-error

.PHONY: all clean cleanall open quick

# Default target
all: $(MAIN).pdf

# Build the PDF (run pdflatex -> bibtex -> pdflatex -> pdflatex)
$(MAIN).pdf: $(MAIN).tex $(MAIN).bib
	@echo "Building $(MAIN).pdf..."
	$(LATEX) $(LATEX_FLAGS) $(MAIN).tex
	$(BIBTEX) $(MAIN)
	$(LATEX) $(LATEX_FLAGS) $(MAIN).tex
	$(LATEX) $(LATEX_FLAGS) $(MAIN).tex
	@echo "Build complete: $(MAIN).pdf"

# Quick build (single pdflatex pass, useful for drafts)
quick: $(MAIN).tex
	@echo "Quick building $(MAIN).pdf..."
	$(LATEX) $(LATEX_FLAGS) $(MAIN).tex

# Clean auxiliary files
clean:
	@echo "Cleaning auxiliary files..."
	rm -f *.aux *.log *.out *.bbl *.blg *.toc *.lof *.lot *.fls *.fdb_latexmk *.synctex.gz

# Clean everything including the PDF
cleanall: clean
	@echo "Removing PDF..."
	rm -f $(MAIN).pdf

# Open the PDF (Linux)
open: $(MAIN).pdf
	@if command -v xdg-open > /dev/null; then \
		xdg-open $(MAIN).pdf; \
	elif command -v evince > /dev/null; then \
		evince $(MAIN).pdf; \
	else \
		echo "No PDF viewer found"; \
	fi

